UMIX: Improving Importance Weighting for Subpopulation Shift via Uncertainty-Aware Mixup

Subpopulation shift widely exists in many real-world machine learning applications, referring to the training and test distributions containing the same subpopulation groups but varying in subpopulation frequencies. Importance reweighting is a normal way to handle the subpopulation shift issue by imposing constant or adaptive sampling weights on each sample in the training dataset. However, some recent studies have recognized that most of these approaches fail to improve the performance over empirical risk minimization especially when applied to over-parameterized neural networks. In this work, we propose a simple yet practical framework, called uncertainty-aware mixup (UMIX), to mitigate the overfitting issue in over-parameterized models by reweighting the ''mixed'' samples according to the sample uncertainty. The training-trajectories-based uncertainty estimation is equipped in the proposed UMIX for each sample to flexibly characterize the subpopulation distribution. We also provide insightful theoretical analysis to verify that UMIX achieves better generalization bounds over prior works. Further, we conduct extensive empirical studies across a wide range of tasks to validate the effectiveness of our method both qualitatively and quantitatively. Code is available at https://github.com/TencentAILabHealthcare/UMIX.

==> 3_preliminaries.tex <==
The necessary background and notations  are provided in this section. Given $N$ training samples $\mathcal{D}=\{(x_i, y_i)\}_{i=1}^{N}$, where $x\in\mathcal{X}$, $y\in \mathcal{Y}$ are the input and label respectively, we consider the setting that there are $G$ predefined groups (subpupulations) and each group is a subset of $\mathcal{D}$ with $N^g$ samples, i.e., $\mathcal{D}_g=\{(x_{i}^{g}, y_{i}^{g})\}_{i=1}^{N_g}$. Our goal is to obtain a model $f_{\theta}: \mathcal{X}\rightarrow \mathcal{Y}$ parameterized by $\theta \in \Theta$ that performs well on all subpopulations. The empirical risk minimization (ERM) algorithm minimizes the expected risk $\mathbb{E}{[\ell(f_\theta(x_i),y_i)]}$ without considering the group information, where $\ell$ denotes the loss function. Unfortunately, when trained with ERM, the model pays more attention to the majority subpopulations in the training set, resulting in poor performance on the minority subpopulations. For example, the ERM-based models may learn spurious correlations that exist in majority subpopulations but not in minority subpopulations \cite{Sagawa2020Distributionally}. The proposed method aims to learn models that are robust to distributional shift by importance weighting.

\textbf{Group-Aware vs Group-Oblivious.} Some previous works have assumed that the group information is available during training. This is called the group-aware setting. However, due to some reasons (e.g., privacy reasons), we may not have training group information. This paper studies the group-oblivious setting, which cannot obtain group information for each example at training time. This requires the model to be able to perceive poorly performing samples and pay more attention to them.
